Constant-Memory Differentiable Light Tracing

Reverse-mode differentiation of Monte Carlo light transport naively stores a computation graph that grows with path length, ruling it out for deep or high-sample simulation. Path Replay Backpropagation (PRB) removes that cost for viewpoint path tracing by reconstructing paths from their seeds and replaying them backward in constant memory. The construction rests on a one-path-one-pixel property that light tracing lacks: one light path contributes to many pixels, and its per-vertex adjoints cannot be recovered during replay from constant-size state. We show this prevents a direct extension of PRB, and that buffering the per-vertex data stays linear in path length. We then evaluate two constant-memory formulations. Reservoir Light Replay Backpropagation compresses a path's sensor connections into one representative by weighted reservoir sampling, keeping two passes at the cost of a sampling decision. LRB-3-pass adds a traversal that accumulates downstream adjoints first, keeping every connection and matching naive automatic differentiation in expectation. Both support differentiating with fixed or parameter-dependent path sampling (detached and attached), and both extend to participating media. We validate against naive AD and finite differences, characterize the memory and runtime trade-offs, and recover specular and volumetric caustics by light tracing alone.

==> figures/tikz/diagram-fonts.tex <==
% Fonts matching acmart (Libertine text, newtxmath), for the standalone
% wrappers only; the paper loads these through acmart.
\usepackage[T1]{fontenc}
\usepackage[tt=false, type1=true]{libertine}
\usepackage[libertine]{newtxmath}


==> figures/tikz/lrb-scene.tex <==
% Common scene for the LRB-3-pass figure: image plane, three surfaces,
% the emitter and the light path emitter -> x1 -> x2 -> x3.
% Hatched pixels: x1 -> (1,3), x2 -> (4,4), x3 -> (3,1).
% \lrbscene draws one row; call it inside a shifted scope.
\newcommand{\lrbscene}{%
  \coordinate (X1) at (704.6,48.7);
  \coordinate (X2) at (527.7,268.8);
  \coordinate (X3) at (390.8,54.5);
  \coordinate (E)  at (830.4,234.8);
  \lrbscreen
  \hatchpx{1}{3}\hatchpx{4}{4}\hatchpx{3}{1}
  \screenlines
  \surf{(527.2,308.6)}{(438.2,253.9)}{(600.8,234.8)}
  \surf{(799.8,97.1)}{(616.1,51.2)}{(715.6,5.3)}
  \surf{(463.1,58.8)}{(317.7,81.8)}{(391.4,22.8)}
  \lrbsun{(861,273.1)}
}
\newcommand{\lightpaths}{%
  \draw[lightpath] (E)  -- (X1);
  \draw[lightpath] (X1) -- (X2);
  \draw[lightpath] (X2) -- (X3);
}
\newcommand{\vertices}{%
  \vtx{(X1)}\vtx{(X2)}\vtx{(X3)}
  \node[lbl, anchor=base east] at (698,26) {$x_1$};
  \node[lbl, anchor=base west] at (511,282) {$x_2$};
  \node[lbl, anchor=base east] at (384,2) {$x_3$};
}
\newcommand{\adjointreads}{%
  \draw[adjoint, shorten >=3pt] (px-4-4) -- (X2);
  \draw[adjoint, shorten >=3pt] (px-1-3) -- (X1);
  \draw[adjoint, shorten >=3pt] (px-3-1) -- (X3);
  \node[lbl, anchor=base west] at (300,246) {$\bar{L}_2$};
  \node[lbl, anchor=base west] at (373,140) {$\bar{L}_1$};
  \node[lbl, anchor=base west] at (245,100) {$\bar{L}_3$};
}
% row title, top left
\newcommand{\passtitle}[1]{%
  \node[font=\lblnote\bfseries, anchor=base west, inner sep=0pt] at (190,300) {#1};}

